High-level Counterexamples for Probabilistic Automata

Providing compact and understandable counterexamples for violated system properties is an essential task in model checking. Existing works on counterexamples for probabilistic systems so far computed either a large set of system runs or a subset of the system's states, both of which are of limited use in manual debugging. Many probabilistic systems are described in a guarded command language like the one used by the popular model checker PRISM. In this paper we describe how a smallest possible subset of the commands can be identified which together make the system erroneous. We additionally show how the selected commands can be further simplified to obtain a well-understandable counterexample.

==> Makefile <==
.PHONY: default clean distclean


default: main.pdf


main.pdf: *.tex literature.bib macros.sty
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main


clean:
	rm -f *.aux *.log *.bbl *.blg *~

distclean: clean
	rm -f main.pdf


==> table_results.tex <==
\begin{footnotesize}
\scalebox{0.8}{%
\addtolength{\tabcolsep}{0.1pt}
\begin{tabular}{lrrcrrr@{\quad}crrr@{\quad}crrr@{\quad}rr}
  \toprule
                    & \multicolumn{6}{c}{no cuts} & \multicolumn{4}{c}{all cuts} & \multicolumn{4}{c}{best cut combination} & \multicolumn{2}{c}{branches} \\  \cmidrule(lr){2-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}\cmidrule(lr){16-17}
  Model             & Var. & Constr. & {Time} & Mem.   & $n$ & lb  & {Time} & Mem. & $n$ & lb & {Time} & Mem. & $n$ & lb  & simp. & $|S'|$ \\
  \midrule
  coin-2-1          & 277  & 491     & \TO &	773 &	9 &	8 &	298.56 & 	146 &	9 &	\opt 	 & 145.76 & 95 & 9 & \opt    & 1/12 & 28 \\
  coin-2-2          & 533  & 1004    & \TO &	864 &	9 &	6 &	\TO &	676 &	9 &	7 	         & \TO    & 562 & 9 & 7 & 1/12 & 72 \\
  coin-2-4          & 1045 & 2028    & \TO &	511 &	9 &	6 &	\TO &	162 &	9 &	6 	         & \TO    & 426 & 9 & 7 & 1/12 & 105 \\
  coin-2-5          & 1301 & 2540    & \TO &	485 &	9 &	5 &	\TO &	121 &	9 &	6 	         & \TO    & 408 & 9 & 6 & 1/12 & 165 \\
  coin-2-6          & 1557 & 3052    & \TO &	550 &	9 &	5 &	\TO &	159 &	9 &	6 	         & \TO    & 495 & 9 & 6 & 1/12 & 103 \\
  coin-4-1          & 26767 & 50079  & \TO &	642 &	\novalue &3 &	\TO &	627&	20 &	3 	 & \TO    & 703 & 20 & 5 & 2/24 & 391 \\
  coin-4-2          & 47759 & 92063  & \TO &	947 &	\novalue &3 &	\TO &	993&	\novalue &	3 	  & \TO & 961 & \novalue & 4 & \novalue & \multicolumn{1}{c}{??} \\[.7ex]%\arrayrulecolor{gray!50}\hline\arrayrulecolor{black}
  csma-2-2          & 2123 & 5990    & 2.49 &	 24 &	32 &	\opt &	17.88 & 	50 &	32 &	\opt 	         & 2.11   & 24 & 32 & \opt & 3/42 & 879 \\
  csma-2-4          & 15977 & 46882  & 195.39 &	208 &	36 &	\opt &	263.89 & 	397 &	36 &	\opt     & 184.05 & 208 & 36 & \opt & 20/90  & 4522 \\[.7ex]%\arrayrulecolor{gray!50}\hline\arrayrulecolor{black}
  fw-1        & 3974 & 13121   & \TO &	205 &	28 &	27 &	184.49 & 	119 &	28 &	\opt 	 & 44.21 & 135 & 28 & \opt & 38/68 & 419 \\
%  firewire-2        & 6632 & 22054   & \TO &	191 &	28 &	26 &	\TO &	248 &	28 &	25 	 & 63.65 & 184 & 28 & \opt & 38/68 & 432 \\
  fw-4        & 13144 & 43836  & \TO &	268 &	28 &	21 &	\TO &	367 &	28 &	21 	 & 107.71 & 328 & 28 & \opt & 38/68 & 424 \\
  fw-10       & 46282 & 153764 & \TO &	790 &	28 &	13 &	\TO &	1141 &	28 &	18  & 545.68 & 993 & 28 & \opt & 38/68 & 428 \\
  fw-15       & 96222 & 318579 & \TO &	1496&28 &	9  &	\TO &	958 &	31 &	14 	 & \TO & 1789 & 28 & 18 & 33/68 & 416 \\[.7ex]%\arrayrulecolor{gray!50}\hline\arrayrulecolor{black}
%  wlan-0-1          & 3064  & 192    & 0.02 &	9 &	8 &	\opt &	0.05 & 	10 &	8 &	\opt 	 & 0.02 & 9 & 8 & \opt & 6/14 & 7 \\
  wlan-0-2          & 7072  & 6602   & \TO &	324 &	33 &	15 &	\TO &	209 &	33 &	30 	 & \TO & 174 & 33 & 32 & 23/72 & 3178\\
  wlan-0-5          & 19012 & 25808  & \TO &	570 &	\novalue & 10 &	\TO &	351 &	\novalue &	30	 & \TO & 357 & \novalue & 30 & \novalue & \multicolumn{1}{c}{??} \\
  wlan-2-1          & 28538 & 192    & 0.04 &	43 &	8 &	\opt &	0.07 & 	44 &	8 &	\opt 	 & 0.04 & 43 & 8 & \opt & 6/14 & 7 \\
  wlan-2-2          & 29607 & 15768  & \TO &	413 &	33 &	14 &	\TO &	188 &	33 &	30 	 & \TO & 180 & 33 & 30 & 23/72 & 25708 \\
  wlan-2-3          & 36351 & 18922  & \TO &	600 &	38 &	14 &	\TO &	315 &	37 &	32 	 & \TO & 275 & 38 & 32 & 31/72 &  25173 \\
  wlan-3-1          & 96360 & 192    & 0.09 &	137 &	8 &	\opt &	0.13 & 	137 &	8 &	\opt 	 & 0.08 & 137 & 8 & \opt & 6/14 & 7 \\
  wlan-3-2          & 97429 & 6602   & \TO &	450 &	33 &	15 &	\TO &	292 &	33 &	30 	 & \TO & 260 & 33 & 31 & 23/72 & 93639\\
  \bottomrule
\end{tabular}}
\end{footnotesize}

